DeformSyncNet: Deformation Transfer via Synchronized Shape Deformation Spaces

Shape deformation is an important component in any geometry processing toolbox. The goal is to enable intuitive deformations of single or multiple shapes or to transfer example deformations to new shapes while preserving the plausibility of the deformed shape(s). Existing approaches assume access to point-level or part-level correspondence or establish them in a preprocessing phase, thus limiting the scope and generality of such approaches. We propose DeformSyncNet, a new approach that allows consistent and synchronized shape deformations without requiring explicit correspondence information. Technically, we achieve this by encoding deformations into a class-specific idealized latent space while decoding them into an individual, model-specific linear deformation action space, operating directly in 3D. The underlying encoding and decoding are performed by specialized (jointly trained) neural networks. By design, the inductive bias of our networks results in a deformation space with several desirable properties, such as path invariance across different deformation pathways, which are then also approximately preserved in real space. We qualitatively and quantitatively evaluate our framework against multiple alternative approaches and demonstrate improved performance.

==> sections/related_work_list.tex <==
% !TEX root = ../paper.tex

\section{Related Work}
\label{sec:related_work}



%%%%
\subsection{3D Shape Deformation}

> Non-neural-net methods
(Cannot learn plausibility in a data-driven way)
Survey: On Linear Variational Surface Deformation Methods~\cite{Botsch:2008}

> Generative models (do not *deform* input shape but just decode a new shape)
    >> Voxels
    Learning a probabilistic latent space object shapes~\cite{Wu:2016}
    and more...
    
    >> Point clouds
    Point cloud GAN~\cite{Achlioptas:2019}, Tree-based~\cite{Shu:2019}
    
    >>  Parts
    GRASS~\cite{Li:2017}
    SDM-NET~\cite{Gao:2019}
    StructureNet~\cite{Mo:2019:StructureNet}
    SAGNet~\cite{Wu:2019}
    CompoNet: Learning to Generate the Unseen by Part Synthesis and Composition~\cite{Schor:2019}

> Neural-Net-based
    >> Voxel-based offset representation (Limited to voxel resolution)
    Deformation Flows~\cite{Yumer:2016}
    Learning Free-Form Deformations for 3D Object Reconstruction~\cite{Jack:2018}
    DeformNet: Free-Form Deformation Network for 3D Shape Reconstruction from a Single Image~\cite{Kurenkov:2018}
    ALIGNet~\cite{Hanocka:2018}

    >> Taking meshes as input (Specialized for organic shapes)
    MeshVAE~\cite{Tan:2018a}
    Deformable Shape Completion with Graph Convolutional Autoencoders~\cite{Litany:2018}
    Mesh-based Autoencoders for Localized Deformation Component Analysis~\cite{Tan:2018b}
    3D-CODED~\cite{groueix20183d}

    >> Taking sampled points as input (We show better fitting accuracy and enable deformation transfer)
    Cycle Consistency~\cite{CycleConsistency}
    3DN~\cite{3DN}
    DiscoNet~\cite{Mehr:2019}

    >> Neural Cages~\cite{NeuralCages}



%%%%
\subsection{Structure-Aware 3D Shape Editing}

> Single shape analysis\\
    >> Preserving local geometries
    Non-homogeneous Resizing of Complex Models~\cite{Kraevoy:2008}
    
    >> Global structure
        >>> Orthogonality, Parallelism
        iWIRES: An Analyze-and-Edit Approach to Shape Manipulation~\cite{Gal:2009}
        Component-wise Controllers for Structure-Preserving Shape Manipulation~\cite{Zheng:2011}
        >>> Symmetry
        Symmetry Hierarchy of Man‐Made Objects~\cite{Wang:2011}
        >>> Articulation of Parts
        Joint-aware Manipulation of Deformable Models~\cite{Xu:2009}

> Shape collection analysis\\
    >> No explicit understanding of correlation of handles
    Maks' SIGGRAPH 11'~\cite{Ovsjanikov:2011}\\
    
    >> Require correspondences
    Meta-representation~\cite{Fish:2014}
    
    >> Find templates - Hard to apply to a diverse family of shapes, or can only analyze high-level parts.
    Vova's SIGGRAPH 13' (Template)~\cite{Kim:2013}
    Recurring Part Arrangements~\cite{Zheng:2014}
    Co-Constrained Handles~\cite{Yumer:2014}




%%%%
\subsection{Deformation Transfer}

> Seminal work!
Deformation Transfer for Triangle Meshes~\cite{Sumner:2004}

> Requires correspondences\\
    >> Point-wise dense correspondences
    Deformation Transfer for Triangle Meshes~\cite{Sumner:2004}
    Example-based Deformation Transfer for 3D Polygon Models~\cite{Chu:2010}
    >>> Intra-class correspodences
    CycleMeshVAE~\cite{Gao:2018}

    >> Keypoints
    Deformation Transfer to Multi-Component Objects~\cite{Zhou:2010}
    Biharmonic deformation transfer with automatic key point selection~\cite{Yang:2018}

    >> Cages
    Spatial Deformation Transfer~\cite{Ben-Chen:2009}
    Cage-based deformation transfer~\cite{Chen:2010}

    >> Parts
    Semantic Deformation Transfer~\cite{Baran:2009}

> Style Transfer (Requires correspondences)
Analogy-Driven 3D Style Transfer~\cite{Ma:2014}
Style-Content Separation by Anisotropic Part Scales~\cite{Xu:2010}

> Motion retargetting (Requires correspondences)
Realtime Style Transfer for Unlabeled Heterogeneous Human Motion~\cite{Xia:2015}
Neural kinematic networks for unsupervised motion retargetting~\cite{Villegas:2018}

> Shape Analogies
(Mention 'Image analogies')
    >> Shape differences, Retrieval  (Not *deforming* the input shape), Requires functional correspondences.
    Map-based exploration of intrinsic shape differences and variability~\cite{Rustamov:2013}
    Functional characterization of intrinsic extrinsic geometry~\cite{Corman:2017}

    >> Decoding from Shape latent space (Not *deforming* the input shape)\\
    Learning a probabilistic latent space object shapes~\cite{Wu:2016}
    LOGAN~\cite{Yin:2019}

> StructEdit~\cite{Mo:2019:StructEdit}
Topological change transfer


==> tables/deform_and_transfer_box.tex <==
\begin{table}[t!]
\caption{}
\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
{\small
%\setlength\tabcolsep{2pt}
\begin{tabularx}{\columnwidth}{>{\centering}m{1.1cm}|>{\centering}m{0.9cm}|*{5}Y}
\toprule
  \multicolumn{2}{c|}{Category} & Airplane & Car & Chair & Sofa & Table\\
\midrule
  \multirow{5}{*}{\shortstack{Fitting\\CD\\($\times 10^{-3}$)\\$\downarrow$ is better}}
  & ICP & 3.13 & \textbf{2.40} & 11.57 & 9.32 & 15.85 \\ 
  & 3DN & \textbf{3.04} & 5.90 & 7.18 & 4.29 & 8.85 \\ 
  & CC & 25.57 & 16.88 & \textbf{3.38} & \textbf{2.73} & \textbf{3.66} \\ 
  & NC & 4.90 & 5.50 & 7.63 & 3.59 & 9.99 \\ 
  & \DSN & 4.78 & 4.34 & 8.14 & 4.85 & 14.45 \\ 
  & Concat$^\ast$ & 3.52 & 3.49 & 6.58 & 3.73 & 10.37 \\
% \midrule
%   \multirow{5}{*}{\shortstack{\footnotesize{Consistency}\\CD\\($\times 10^{-3}$)\\$\downarrow$ is better}}
%   & ICP &  &  &  &  & \\
%   & 3DN &  &  &  &  & \\
%   & CC &  &  &  &  & \\
%   & NC &  &  &  &  & \\
%   & \DSN &  &  &  &  & \\
%   & Concat$^\ast$ &  &  &  &  & \\
\midrule
  \multirow{5}{*}{\shortstack{MMD-CD\\($\times 10^{-3}$)\\$\downarrow$ is better}}
  & 3DN & 1.48 & \textbf{1.87} & 8.65 & 3.11 & 13.27 \\ 
  & CC & 2.27 & 9.68 & 12.54 & 6.25 & 19.63 \\ 
  & NC & 1.48 & 3.70 & 7.48 & 3.32 & 6.99 \\ 
  & \DSN & \textbf{1.08} & 2.32 & \textbf{5.98} & \textbf{2.73} & \textbf{5.74} \\ 
  & Concat$^\ast$ & 1.69 & 4.13 & 11.15 & 3.89 & 8.86 \\
\midrule
  \multirow{5}{*}{\shortstack{Cov-CD\\(\%)\\$\uparrow$ is better}}
  & 3DN & 30.9 & 27.0 & 28.4 & 33.9 & 23.8 \\ 
  & CC & 17.4 & 13.9 & 18.8 & 19.0 & 16.8 \\ 
  & NC & 36.1 & 19.2 & 34.2 & 36.2 & 35.4 \\ 
  & \DSN & \textbf{38.9} & \textbf{35.3} & \textbf{39.8} & \textbf{42.8} & \textbf{43.2} \\ 
  & Concat$^\ast$ & 22.2 & 15.9 & 16.6 & 17.3 & 25.9 \\  
\bottomrule
\end{tabularx}
}
\label{tbl:deform_and_transfer_box}
\end{table}


==> tables/project_SynTable.tex <==
\begin{table}[t!]
\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
{\small
%\setlength\tabcolsep{2pt}
\begin{tabularx}{\columnwidth}{>{\centering}m{1.9cm}|*{4}Y}
\toprule
  Constraints & Leg x scale symmetry & Leg y scale symmetry & Leg z scale symmetry & z contacting\\
\midrule
  MAE & 0.0072 & 0.0052 & 0.0052 & 0.0238 \\ 
  Ref scale & \multicolumn{4}{c}{0.3750} \\
\bottomrule
\end{tabularx}
}
\label{tbl:project_syn}
\end{table}

==> tables/tables.tex <==

\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
{\small
%\setlength\tabcolsep{2pt}
\begin{tabularx}{\columnwidth}{>{\centering}m{1.1cm}|>{\centering}m{0.9cm}|*{5}Y}
\toprule
  \multicolumn{2}{c|}{Category} & Airplane & Car & Chair & Lamp & Table\\
\midrule
  \multirow{5}{*}{\shortstack{Fitting\\CD\\($\times 10^{-3}$)\\$\downarrow$ is better}}
  & NR-ICP &  &  &  &  & \\
  & 3DN & 6.32 & 2.54 & 8.51 & 5.04 & 14.15 \\ 
  & CC & 9.81 & 3.26 & 14.61 & 4.18 & 30.65 \\ 
  & NC & 18.82 & 6.73 & 25.80 & 7.49 & 41.40 \\ 
  & \textbf{DSN} & 7.17 & 2.20 & 8.00 & 4.58 & 13.88 \\
  & Concat$^\ast$ &  &  &  &  & \\
\midrule
  \multirow{5}{*}{\shortstack{mIoU\\(\%)\\$\uparrow$ is better}}
  & NR-ICP &  &  &  &  & \\
  & 3DN & 58.1 & 58.4 & 46.6 & 48.3 & 45.9 \\ 
  & CC & 77.6 & 67.8 & 65.4 & 61.1 & 65.6 \\ 
  & NC & 78.2 & 67.5 & 66.9 & 61.2 & 64.7 \\ 
  & \textbf{DSN} & 77.6 & 68.2 & 65.6 & 62.2 & 64.9 \\
  & Concat$^\ast$ &  &  &  &  & \\
\midrule
  \multirow{5}{*}{\shortstack{\footnotesize{Consistency}\\CD\\($\times 10^{-3}$)\\$\downarrow$ is better}}
  & ICP &  &  &  &  & \\
  & 3DN &  &  &  &  & \\
  & CC &  &  &  &  & \\
  & NC &  &  &  &  & \\
  & \textbf{DSN} &  &  &  &  & \\
  & Concat$^\ast$ &  &  &  &  & \\
\midrule
  \multirow{5}{*}{\shortstack{MMD-CD\\($\times 10^{-3}$)\\$\downarrow$ is better}}
  & AE &  &  &  &  & \\
  & 3DN & 56.18 & 13.31 & 107.14 & 8.15 & 116.95 \\ 
  & CC & 26.83 & 7.44 & 53.39 & 6.45 & 56.89 \\ 
  & NC & 21.93 & 6.10 & 33.16 & 4.96 & 52.07 \\ 
  & \textbf{DSN} & 23.16 & 6.69 & 31.22 & 5.54 & 45.60 \\
  & Concat$^\ast$ &  &  &  &  & \\
\midrule
  \multirow{5}{*}{\shortstack{COV-CD\\(\%)\\$\uparrow$ is better}}
  & AE &  &  &  &  & \\
  & 3DN & 6.6 & 16.0 & 10.0 & 6.9 & 8.1 \\ 
  & CC & 30.9 & 30.3 & 25.7 & 14.1 & 27.6 \\ 
  & NC & 39.5 & 30.6 & 35.9 & 37.5 & 32.3 \\ 
  & \textbf{DSN} & 40.0 & 29.5 & 36.7 & 33.5 & 33.0 \\ 
  & Concat$^\ast$ &  &  &  &  & \\
\bottomrule
\end{tabularx}
}
\caption{Comparisons among Non-rigid ICP (NR-ICP)~\cite{}, 3DN~\cite{3DN}, Cycle Consistency (CC)~\cite{CycleConsistency}, Neural Cages (NC)~\cite{NeuralCages}, and our DeformSyncNet (DSN). }
\label{tbl:raw_point_clouds}
\end{table}
